Defending Object Detectors against Patch Attacks with Out-of-Distribution Smoothing

Patch attacks against object detectors have been of recent interest due to their being physically realizable and more closely aligned with practical systems. In response to this threat, many new defenses have been proposed that train a patch segmenter model to detect and remove the patch before the image is passed to the downstream model. We unify these approaches with a flexible framework, OODSmoother, which characterizes the properties of approaches that aim to remove adversarial patches. This framework naturally guides us to design 1) a novel adaptive attack that breaks existing patch attack defenses on object detectors, and 2) a novel defense approach SemPrior that takes advantage of semantic priors. Our key insight behind SemPrior is that the existing machine learning-based patch detectors struggle to learn semantic priors and that explicitly incorporating them can improve performance. We find that SemPrior alone provides up to a 40% gain, or up to a 60% gain when combined with existing defenses.

==> tables/diff_approx.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llc|cccc@{}}
\centering
\caption{We find that the native form of \defense is much more robust than its differential approximations. This shows that the ML-based differential approximations struggled to replicate these OOD oracles.}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Defense}}} & \multirow{2}{*}{\textbf{Clean}} & \multicolumn{4}{c}{\textbf{Adaptive Attack}}                                                                     \\ \cmidrule(l){4-7} 
\multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                                  &                                 & \textbf{75 x 75} & \textbf{100 x 100} & \multicolumn{1}{c|}{\textbf{125 x 125}} & \multicolumn{1}{l}{CARLA Mask} \\ \midrule
\textbf{COCO}                                         & \textbf{OURS}                                         & 0.569                           & 0.342            & 0.224              & \multicolumn{1}{c|}{0.216}              & -                              \\
                                                      & \textbf{OURS-DIFF}                                    & 0.616                           & 0.106            & 0.017              & \multicolumn{1}{c|}{0.036}              & -                              \\ \cmidrule(r){1-6}
\textbf{VOC}                                          & \textbf{OURS}                                         & 0.760                           & 0.558            & 0.421              & \multicolumn{1}{c|}{0.421}              & -                              \\
\textbf{}                                             & \textbf{OURS-DIFF}                                    & 0.764                           & 0.134            & 0.018              & \multicolumn{1}{c|}{0.002}              & -                              \\ \cmidrule(r){1-6}
\textbf{CARLA}                                        & \textbf{OURS}                                         & 0.316                           & -                & -                  & \multicolumn{1}{c|}{-}                  & 0.316                          \\
                                                      & \textbf{OURS-DIFF}                                    & 0.342                           & -                & -                  & \multicolumn{1}{c|}{-}                  & 0.025                          \\ \bottomrule
\end{tabular}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{lllllll}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Defense}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{No Attack}}} & \multicolumn{4}{c}{\textbf{Adaptive Attack}}                                                                                            \\ \cline{4-7} 
% \multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                                  & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c}{\textbf{75 x 75}} & \multicolumn{1}{c}{\textbf{100 x 100}} & \multicolumn{1}{c|}{\textbf{125 x 125}} & CARLA Mask    \\ \hline
% \textbf{COCO}                                         & \textbf{OURS}                                         &                                                          &                                      &                                        &                                         &               \\
%                                                       & \textbf{OURS-DIFF}                                    & \multicolumn{1}{l|}{}                                    & 0.065 / 0.106                        & 0.010 / 0.017                          & 0.022 / 0.036                           &               \\ \cline{1-6}
% \textbf{VOC}                                          & \textbf{OURS}                                         & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c}{}                 & \multicolumn{1}{c}{}                   & \multicolumn{1}{c}{}                    &               \\ \cline{1-1}
% \textbf{}                                             & \textbf{OURS-DIFF}                                    & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c}{0.074 / 0.134}    & \multicolumn{1}{c}{0.009 / 0.018}      & \multicolumn{1}{c}{0.001 / 0.002}       &               \\ \cline{1-6}
% \textbf{CARLA}                                        & \textbf{OURS}                                         &                                                          &                                      &                                        &                                         &               \\
%                                                       & \textbf{OURS-DIFF}                                    &                                                          &                                      &                                        &                                         & 0.013 / 0.025
% \end{tabular}
% \end{table}

==> tables/existing_defenses.tex <==
% \begin{table*}[]
% \centering
% \caption{Caption}\label{tab:existing_defenses}

% \scalebox{0.7}{\begin{tabular}{@{}l|l|ccc|ccc|ccc@{}}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Defense}}} & \multicolumn{3}{c|}{\textbf{Orig. Attack}}                                           & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Orig. Attack\\ 1000 Steps\end{tabular}}} & \multicolumn{3}{c}{\textbf{Our Attack}}                                              \\ \cmidrule(l){3-11} 
% \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\textbf{75}} & \multicolumn{1}{c|}{\textbf{100}} & \textbf{125}  & \multicolumn{1}{c|}{\textbf{75}}     & \multicolumn{1}{c|}{\textbf{100}}     & \textbf{125}     & \multicolumn{1}{c|}{\textbf{75}} & \multicolumn{1}{c|}{\textbf{100}} & \textbf{125}  \\ \midrule
% \textbf{COCO}                                          & \textbf{SAC}                                           & 0.313 / 0.537                    & 0.335 / 0.536                     & 0.280 / 0.457 & Running                              & 0.163 / 0.257                         & Running          & 0.079 / 0.124                    & 0.038 / 0.062                     & running       \\ \midrule
% \multirow{2}{*}{\textbf{VOC}}                          & \textbf{SAC}                                           & Running                          & Running                           & Running       & Running                              & 0.235 / 0.389                         & Running          & 0.065 / 0.116                    & Need to run transfer              & 0.020 / 0.043 \\
%                                                        & \textbf{PZ}                                            & 0.442 / 0.727                    & 0.392 / 0.689                     & 0.353 / 0.645 & not started                          & not started                           & not started      & running                          & 0.040 / 0.070                     & running       \\ \bottomrule
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Caption}\label{tab:existing_defenses}
\begin{tabular}{@{}l|l|c|ccc|ccc|ccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Defense}}} & \multirow{2}{*}{\textbf{No Attack}} & \multicolumn{3}{c|}{\textbf{Orig. Attack}}                                                           & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Orig. Attack\\ 1000 Steps\end{tabular}}}      & \multicolumn{3}{c}{\textbf{Our Attack}}                                                              \\ \cmidrule(l){4-12} 
\multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                  &                                     & \multicolumn{1}{c|}{\textbf{75 x 75}} & \multicolumn{1}{c|}{\textbf{100 x 100}} & \textbf{125 x 125} & \multicolumn{1}{c|}{\textbf{75 x 75}} & \multicolumn{1}{c|}{\textbf{100 x 100}} & \textbf{125 x 125} & \multicolumn{1}{c|}{\textbf{75 x 75}} & \multicolumn{1}{c|}{\textbf{100 x 100}} & \textbf{125 x 125} \\ \midrule
\textbf{COCO}                                          & \textbf{SAC}                                           & 0.398 / 0.618                       & \multicolumn{1}{c|}{0.313 / 0.537}    & \multicolumn{1}{c|}{0.335 / 0.536}      & 0.280 / 0.457      & \multicolumn{1}{c|}{0.201/ 0.308}     & \multicolumn{1}{c|}{0.163 / 0.257}      & 0.178 / 0.288      & \multicolumn{1}{c|}{0.079 / 0.124}    & \multicolumn{1}{c|}{0.038 / 0.062}      & 0.037 / 0.062      \\ \midrule
\multirow{2}{*}{\textbf{VOC}}                          & \textbf{SAC}                                           & 0.482 / 0.767                       & \multicolumn{1}{c|}{0.436 / 0.705}    & \multicolumn{1}{c|}{0.389 / 0.662}      & 0.341 / 0.610      & \multicolumn{1}{c|}{0.201 / 0.308}    & \multicolumn{1}{c|}{0.235 / 0.389}      & 0.199 / 0.358      & \multicolumn{1}{c|}{0.065 / 0.116}    & \multicolumn{1}{c|}{0.008 / 0.016}      & 0.020 / 0.043      \\
                                                       & \textbf{PZ}                                            & 0.482 / 0.767                       & \multicolumn{1}{c|}{0.442 / 0.727}    & \multicolumn{1}{c|}{0.392 / 0.689}      & 0.353 / 0.645      & \multicolumn{1}{c|}{not started}      & \multicolumn{1}{c|}{not started}        & not started        & \multicolumn{1}{c|}{running}          & \multicolumn{1}{c|}{0.040 / 0.070}      & 0.020 / 0.039      \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/existing_defenses_0.5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Same format and trend as Table 1, but over mAP @ IoU = 0.5.}\label{tab:existing_defenses_0.5}
\begin{tabular}{@{}llc|ccc|ccc|ccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Def.}}} & \multirow{2}{*}{\textbf{Clean}} & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}$L_{e2e}$\\ <= 200 Steps\end{tabular}}}                 & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}$L_{e2e}$\\ 1000 Steps\end{tabular}}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}$L_{obj\_det} + \lambda L_{patch\_seg}$\\ 1000 Steps\end{tabular}}}                    \\ \cmidrule(l){4-12} 
\multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                                  &                                     & \textbf{75} & \textbf{100} & \textbf{125} & \textbf{75}              & \textbf{100}             & \textbf{125}             & \textbf{75} & \textbf{100} & \textbf{125} \\ \midrule
\textbf{COCO}                                         & \textbf{SAC}                                          & 0.618                               & 0.537            & 0.536              & 0.457              & 0.308                         & 0.257                          & 0.288                          & \textbf{0.124}            & \textbf{0.062}              & \textbf{0.062}              \\ \midrule
\multirow{2}{*}{\textbf{VOC}}                         & \textbf{SAC}                                          & 0.767                               & 0.705            & 0.662              & 0.610              & 0.308                         & 0.389                          & 0.358                          & 0\textbf{.116}            & \textbf{0.016}              & \textbf{0.043}              \\
                                                      & \textbf{PZ}                                           & 0.767                               & 0.727            & 0.689              & 0.645              & 0.703                         & 0.709                          & 0.664                          & \textbf{0.118}            & \textbf{0.070}              & \textbf{0.039}              \\ \bottomrule
\end{tabular}
\end{table}

==> tables/robustness_0.5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Same as Table~\ref{tab:robustness_box} but over mAP @ IoU = 0.5}\label{tab:robustness_0.5}
\begin{tabular}{@{}llc|cccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Defense}}} & \multirow{2}{*}{\textbf{Clean}} & \multicolumn{4}{c}{\textbf{Adaptive Attack}}                                                                              \\ \cmidrule(l){4-7} 
\multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{}                                  &                                 & \textbf{75 x 75} & \textbf{100 x 100} & \multicolumn{1}{c|}{\textbf{125 x 125}} & \multicolumn{1}{l}{\textbf{CARLA Mask}} \\ \midrule
\textbf{COCO}                                         & \textbf{SAC}                                          & 0.618                           & 0.124            & 0.062              & \multicolumn{1}{c|}{0.062}              & -                                       \\
                                                      & \textbf{OURS}                                         & 0.569                           & 0.342            & 0.224              & \multicolumn{1}{c|}{0.216}              & -                                       \\
                                                      & \textbf{OURS + SAC}                                   & 0.568                           & \textbf{0.469}            & \textbf{0.449}              & \multicolumn{1}{c|}{\textbf{0.473}}              & -                                       \\ \midrule
\textbf{VOC}                                          & \textbf{SAC}                                          & 0.767                           & 0.116            & 0.016              & \multicolumn{1}{c|}{0.043}              & -                                       \\
\textbf{}                                             & \textbf{PZ}                                           & 0.767                           & 0.118            & 0.070              & \multicolumn{1}{c|}{0.039}             & -                                       \\
                                                      & \textbf{OURS}                                         & 0.760                           & 0.558            & 0.421              & \multicolumn{1}{c|}{0.421}              & -                                       \\
                                                      & \textbf{OURS + SAC}                                   & 0.760                           & \textbf{0.715}            & \textbf{0.683}              & \multicolumn{1}{c|}{\textbf{0.626}}              & -                                       \\ \bottomrule
\end{tabular}
\end{table}
